Structural Rounding: Approximation Algorithms for Graphs Near an Algorithmically Tractable Class

We develop a new framework for generalizing approximation algorithms from the structural graph algorithm literature so that they apply to graphs somewhat close to that class (a scenario we expect is common when working with real-world networks) while still guaranteeing approximation ratios. The idea is to $\textit{edit}$ a given graph via vertex- or edge-deletions to put the graph into an algorithmically tractable class, apply known approximation algorithms for that class, and then $\textit{lift}$ the solution to apply to the original graph. We give a general characterization of when an optimization problem is amenable to this approach, and show that it includes many well-studied graph problems, such as Independent Set, Vertex Cover, Feedback Vertex Set, Minimum Maximal Matching, Chromatic Number, ($\ell$-)Dominating Set, Edge ($\ell$-)Dominating Set, and Connected Dominating Set. To enable this framework, we develop new editing algorithms that find the approximately-fewest edits required to bring a given graph into one of several important graph classes (in some cases, also approximating the target parameter of the family). For bounded degeneracy, we obtain a bicriteria $(4,4)$-approximation which also extends to a smoother bicriteria trade-off. For bounded treewidth, we obtain a bicriteria $(O(\log^{1.5} n), O(\sqrt{\log w}))$-approximation, and for bounded pathwidth, we obtain a bicriteria $(O(\log^{1.5} n), O(\sqrt{\log w} \cdot \log n))$-approximation. For treedepth $2$ (also related to bounded expansion), we obtain a $4$-approximation. We also prove complementary hardness-of-approximation results assuming $\mathrm{P} \neq \mathrm{NP}$: in particular, these problems are all log-factor inapproximable, except the last which is not approximable below some constant factor ($2$ assuming UGC).

==> positive_results/weak_coloring_lp.tex <==

In this section, we design a bicriteria approximation for the problem of editing a graph $G = (V, E)$ to have bounded weak $\Tc$-coloring number.
Principally, we give an $(O(1), O(1))$-approximation for \bWCNfull which asks for a minimum edit set $\editset$ of either edges or vertices such that $G \setminus \editset$ has weak $\Tc$-coloring number at most $\Tt$ (see Definition~\ref{definition:wcol} for the formal definition).

Remember that by Definition~\ref{definition:wcol}, if the graph $G = (V, E)$ has weak $\Tc$-coloring number at most $\Tt$, then there must exist some ordering $L$ such that $|\wreach{\Tc}{G}{L}{v}| \leq \Tt$ for all $v \in V$.
Our LP formulation works by attempting to construct an ordering and then ensuring that the weak $\Tc$-reachability of every vertex is bounded by $\Tt$ for that ordering.
We use two sets of variables, $x$ and $y$, to enforce a valid partial ordering.
For each ordered pair of vertices $u, v \in V \times V$, $x_{uv} = 1$ if $u$ comes before $v$ in the ordering and zero otherwise.
Additionally, we have a set of variables for every path $T$ in $G$ of length at most $\Tc$.
For each vertex $v \in T$, $y_{Tv} = 1$ if $L(v) \geq L(u)$ for all other $u \in T$ and zero otherwise.
We also need to determine which edges or vertices are edited, and so for each edge $\set{uv} \in E$, $z_{\set{uv}} = 1$ if $\set{uv}$ is in the edit set and zero otherwise
Analagously, for each vertex $v \in V$, $z_v = 1$ if $v$ is in the edit set and zero otherwise.
Finally, for every ordered pair of vertices $u, v \in V \times V$, $P_{uv} = 1$ if $v$ is weakly $\Tc$-reachable from $u$ and zero otherwise.

For simplicity, we will use $C$ to denote the set of all paths in $G$ of length at most $\Tc$ and $C_{uv} \subseteq C$ to denote the set of $uv$-paths in $G$ of length at most $\Tc$.
Note that $|C|$ is bounded polynomially in $|V|$.

\begin{center}
\begin{probbox}{\lpMEWCfull (\lpMEWC)}
	\emph{Input:} \hskip1em $G=(V,E), \Tc, \Tt, w$
\begin{align}
	\text{Minimize} & & \sum_{uv \in E} z_{\set{uv}} w_{\set{uv}} & & \nonumber \\
	\text{s.t.}     & & x_{uv} + x_{vu} &\geq 1 &\forall u, v \in V \times V \label{cst:pair-sum} \\
					& & x_{v_1 v_3} &\leq x_{v_1 v_2} + x_{v_2 v_3} &\forall v_2 \in V, \forall v_1, v_3 \in V \times V \label{cst:no-cycle} \\
					& & y_{Tv} &\leq x_{uv} &\forall u \in T, \forall v \in T, \forall T \in C \label{cst:path-last} \\
					& & \sum_{v \in T} y_{Tv} &\geq 1 &\forall T \in C \label{cst:path-sum} \\
					& & P_{uv} &\geq y_{Tv} - \sum_{pq \in T} z_{\set{pq}} & \forall T \in C_{uv}, \forall u, v \in V \times V \label{cst:hop}\\
					& & \sum_{v \in V} P_{uv} &\leq \Tt & \forall u \in V \label{cst:coloring-number}
\end{align}
\end{probbox}
\end{center}

Note that \lpMEWC given above is specifically for \bWCNE.
The corresponding formulation of \lpMVWC can be derived by simply replacing $z_{\set{uv}}$ for $z_v$ in the objective function and Constraint~\eqref{cst:hop}.

Constraint~\eqref{cst:pair-sum} ensures that a vertex $u$ cannot appear both before and after another vertex $v$.
Constraint~\eqref{cst:no-cycle} make this property transitive so that if $v_3$ appears before $v_2$ and $v_2$ appears before $v_1$, then $v_1$ cannot appear before $v_3$.
Constraint~\eqref{cst:path-last} states that if $v$ comes before any other vertex $u$ in the path $T$, then $v$ cannot be the last vertex in the ordering from $T$.
Since Constraint~\eqref{cst:path-last} allows all $y_{Tv}$ to be set to 0, we add Constraint~\eqref{cst:path-sum} which enforces that one vertex from the path must come last.
Constraint~\eqref{cst:hop} sets $P_{uv} = 1$ if $v$ is weakly $\Tc$-reachable from $u$.
This is the case only if there exists a $uv$-path of length at most $\Tc$ such that every vertex appears before $v$ in the ordering per the definition of weak $\Tc$-reachability in Definition~\ref{definition:wcol}.
If any of the edges or vertices in the path are edited, then the path does not exist in the edited graph, and Constraint~\eqref{cst:hop} will be trivially satisfied even if $P_{uv} = 0$.
Lastly, Constraint~\eqref{cst:coloring-number} ensures that the weak $\Tc$-reachability of every vertex in the edited graph will be at most $\Tt$.

\begin{lemma} \label{lem:weak-lp-relaxation}
\lpMEWCfull and \lpMVWCfull are valid LP-relaxations of \bWCNE and \bWCNV.
\end{lemma}

\begin{proof}
Suppose $\editset$ is a feasible solution for the instance $(G = (V, E), \Tc, \Tt, w)$.
Let $H = G \setminus \editset$.
Since $\wcol{\Tc}{H} \leq \Tt$, there exists an ordering $L$ such that for any vertex $v \in V$, $|\wreach{\Tc}{H}{L}{v}| \leq \Tt$.
Using the ordering $L$, we will construct a feasible solution for \lpMEWC or \lpMVWC whose cost is equal to $w(\editset)$.

First, for each edge $\set{uv} \in E(G)$, we set $z_{\set{uv}} = 1$ if $\set{uv} \in \editset$ and zero otherwise.
Likewise for vertex deletion, for each vertex $v \in V(G)$, we set $z_v = 1$ if $v \in \editset$ and zero otherwise.
Next, we assign values to $x$ and $y$ so that they are consistent with the ordering $L$.
For every ordered pair of vertices $u, v \in V(H) \times V(H)$, we set $x_{uv} = 1$ if $L(u) < L(v)$ and zero otherwise.
Likewise, for each path $T$ in $G$, we find the vertex $v$ such that $L(v) \geq L(u)$ for every other vertex $u \in T$ and set $y_{Tv} = 1$ and zero otherwise.
In the case of vertex deletion, we must also assign values to $x$ and $y$ for vertices in the edit set.
Since the vertices are removed, their location cannot cause any Constraint~\eqref{cst:hop} to be violated.
Thus, we pick an arbitrary ordering $L'$ defined for the vertices in $\editset$ and place them at the beginning of $L$.
To do this, we set $x_{uv} = 1$ and $x_{vu} = 0$ for each $u \in \editset$ and $v \in V(H)$.
Then, for every ordered pair of vertices $u, v \in \editset \times \editset$, we set $x_{uv} = 1$ if $L'(u) < L'(v)$ and zero otherwise.
Finally, for each ordered pair of vertices $u, v \in V \times V$, we set $P_{uv} = 1$ if $v$ is weakly $\Tc$-reachable from $u$ in $H$ according to $L$.
We set $P_{uv} = 0$ in all other cases.
Now, we show that $(x, y, z, P)$ is a feasible solution for \lpMEWC or \lpMVWC depending on the edit operation.

Constraints~\eqref{cst:pair-sum} --~\eqref{cst:path-sum} hold because $x$ and $y$ are constructed from a valid ordering $L$.
Assume that Constraint~\eqref{cst:hop} is violated for some pair of vertices $u, v$ and a $uv$-path $T \in G$ of length at most $\Tc$.
For this to happen, $P_{uv} = 0$, $y_{Tv} = 1$, and $z_{\set{pq}} = 0$ for every $\set{pq} \in T$.
Alternatively, $z_p = 0$ for every $v \in T$ in the case of vertex deletion.
However, this indicates that $T$ must also be in $H$ since no edits were made and that every vertex in $T$ appears before $v$ in the ordering.
This implies that $v$ is weakly $\Tc$-reachable from $u$ though and so $P_{uv}$ must have been set to 1, a contradiction.
Finally, Constraint~\eqref{cst:coloring-number} simply verifies that the weak $\Tc$-reachability of each vertex is at most $\Tt$ and follows from the fact that $\editset$ is a feasible solution.
\end{proof}

Next, we propose a rounding scheme for \lpMEWC.
At a high level, we first find an edit set $\editset$ whose cost is within a constant factor of the optimal fractional solution along with a partial ordering on the vertices of $G$, ensuring that we cannot have undercounted the weak $\Tc$-reachability of any vertex.
Then, we show that no matter how the partial ordering is completed, $\wcol{\Tc}{G \setminus \editset}$ is within a constant factor of $\Tt$.
Although we only give the rounding algorithm for \lpMEWC, it is straightforward to see how it could easily be adjusted for \lpMVWC.

\begin{algorithm}
\caption{Rounding Algorithm for \lpMEWC}\label{alg:weak-coloring-rounding}
\begin{algorithmic}[1]
\Procedure{WeakColoringRounding}{$x, y , z, P$}
\State $\hat{z} \leftarrow z$
\\
\Comment{{\bf Step 1:} Rounding up large $z$}
\ForAll{$z_{\set{uv}} > \eps$}
	\State $\hat{z}_{\set{uv}} \leftarrow 1$
\EndFor
\\
\Comment{{\bf Step 2:} Rounding $x, y$}
\ForAll{$x_{uv}$}
	\If{$x_{uv} < \frac{1}{\Tc}$} \label{line:x-round}
		\State $\hat{x}_{uv} \leftarrow 0$
	\Else
		\State $\hat{x}_{uv} \leftarrow 1$
	\EndIf
\EndFor

\ForAll{$y_{Tv}$} \label{line:y-round}
	\If{$y_{Tv} < \frac{1}{\Tc}$}
		\State $\hat{y}_{Tv} \leftarrow 0$
	\Else
		\State $\hat{y}_{Tv} \leftarrow 1$
	\EndIf
\EndFor

\ForAll{$u, v \in V \times V$} \label{line:p-round}
	\If{There exists $T \in C_{uv}$ such that $\hat{y}_{Tv} > 0$ and $\hat{z}_{\set{pq}} < 1$ for all $\set{pq} \in T$}
		\State $\hat{P}_{uv} \leftarrow 1$
	\Else
		\State $\hat{P}_{uv} \leftarrow 0$
	\EndIf
\EndFor
\\
\Comment{{\bf Step 3:} Rounding down small $z$}
\ForAll{$z_{\set{uv}} \leq \eps$}
	\State $\hat{z}_{\set{uv}} \leftarrow 0$
\EndFor
\State\Return $\hat{\editset} := \set{\set{uv}\in E : \hat{z}_{\set{uv}} = 1}$
\EndProcedure
\end{algorithmic}
\end{algorithm}

\begin{lemma} \label{lem:step-1}
Let $(x,y,z,P)$ be a feasible solution for the \lpMEWC or \lpMVWC instance $(G = (V, E), \Tc, \Tt, w)$.
The solution constructed at the end of step $1$ of Algorithm~\ref{alg:weak-coloring-rounding}, $(x,y,\hat{z},P)$, is a feasible solution for $(G, \Tc, \Tt, w)$ such that $\cost(x,y,\hat{z},P) \leq \frac{1}{\eps} \cdot \cost(x,y,z,P)$.
\end{lemma}

\begin{proof}
Note that for any edge $\set{uv} \in E$, increasing $z_{\set{uv}}$ cannot violate any constraints.
This also applies to increasing $z_v$ for any $v \in V$.
Furthermore, since we only round up $z$ if its value is at least $\eps$, $\hat{z} \leq \frac{1}{\eps} z$.
\end{proof}

Once we set $z_{\set{uv}} = 1$, we can remove each Constraint~\eqref{cst:hop} that contains $z_{\set{uv}}$ and likewise for $z_v$.
Thus, for any remaining constraint, we can assume that $\hat{z}_{\set{uv}} \leq \eps$ for edge deletion and $\hat{z}_v \leq \eps$ for vertex deletion.

\begin{definition} \label{def:beta-feasible-sol}
A solution $(x,y,z,P)$ is \emph{$\beta$-feasible} if it satisfies Constraint~\eqref{cst:pair-sum}, all Constraints~\eqref{cst:path-last} --~\eqref{cst:hop}, and Constraint~\eqref{cst:coloring-number} is not violated by a factor more than $\beta$.
\end{definition}

Note that we allow Constraint~\eqref{cst:no-cycle} to be violated while rounding the solution to the LP.
Since breaking Constraint~\eqref{cst:no-cycle} only allows some $\hat{x}_{uv}$ values to be larger than they ought to be, we will be able to show that the edited graph $G \setminus \hat{\editset}$ must have weak $\Tc$-coloring number bounded by $\beta \Tt$.

\begin{lemma}\label{lem:step-2}
Let $(x,y,z,P)$ be a feasible solution for the \lpMEWC or \lpMVWC instance $(G = (V, E), \Tc, \Tt, w)$.
Assuming $\Tc \eps < \frac{1}{\Tc}$, the solution constructed at the end of step $2$ of Algorithm~\ref{alg:weak-coloring-rounding}, $(\hat{x},\hat{y},\hat{z},\hat{P})$, is a $(\frac{1}{1/\Tc - \Tc \eps})$-feasible solution for $(G, \Tc, \Tt, w)$ such that $\cost(\hat{x},\hat{y},\hat{z},\hat{P}) \leq \frac{1}{\eps} \cdot \cost(x,y,z,P)$.
\end{lemma}

\begin{proof}
By Lemma~\ref{lem:step-1}, $(x,y,\hat{z},P)$ constructed at the end of step $1$ of Algorithm~\ref{alg:weak-coloring-rounding} is a feasible solution with cost at most $\frac{1}{\eps} \cdot \cost(x,y,z,P)$.

It is straightforward to check that Line~\ref{line:x-round} of Algorithm~\ref{alg:weak-coloring-rounding} guarantees that $\hat{x}$ satisfies Constraint~\eqref{cst:pair-sum}.
Likewise, in Constraint~\eqref{cst:path-sum}, at least one variable $y_{Tv}$ must have been greater than $\frac{1}{\Tc}$ or $(x,y,z,P)$ would not have been a feasible solution.
Thus, $y_{Tv}$ must have been rounded up to 1, satisfying Constraint~\eqref{cst:path-sum}.
For Constraint~\eqref{cst:path-last}, since all values of $x$ and $y$ are rounded, the constraint can only be violated if $y_{Tv}$ is rounded up and $x_{uv}$ is rounded down.
However, this implies that $y_{Tv} \geq \frac{1}{\Tc} > x_{uv}$, and so $(x,y,z,P)$ was not a feasible solution, a contradiction.

Constraint~\eqref{cst:hop} can only be violated if $y_{Tv}$ is rounded up.
However, in this case, $\hat{y}_{Tv} < 1$, and so $\hat{P}_{uv} = 1$.
Furthermore, we know $y_{Tv} \geq \frac{1}{\Tc}$.
Also, recall that every $z$ is less than $\eps$ in each remaining constraint.
Thus, $P_{uv} \geq \frac{1}{\Tc} - \Tc \eps$, and so $\hat{P}_{uv} = 1 \leq \frac{P_{uv}}{1/\Tc - \Tc \eps}$.
This inequality also clearly holds in the case where $\hat{P}_{uv}$ is set to 0.

Finally, since we only scaled each $P_{uv}$ up by at most a factor of $\frac{1}{1/\Tc - \Tc \eps}$, we know that for all $u \in V$, $\sum_{v \in V} \hat{P}_{uv} \leq \sum_{v \in V} \frac{P_{uv}}{1/\Tc - \Tc \eps} \leq \frac{\Tt}{1/\Tc - \Tc \eps}$.
Thus, $(\hat{x},\hat{y},\hat{z},\hat{P})$ is a $(\frac{1}{1/\Tc - \Tc \eps})$-feasible solution with cost at most $\frac{1}{\eps} \cdot \cost(x,y,z,P)$.
\end{proof}

Next, we show that by rounding down the values of the coordinates in $\hat{z}$ that are not equal to 1 in step $3$ of Algorithm~\ref{alg:weak-coloring-rounding}, the solution $(\hat{x}, \hat{y}, \hat{z}, \hat{P})$ remains $(\frac{1}{1/\Tc - \Tc \eps})$-feasible solution.

\begin{corollary} \label{cor:step-3}
Let $(x,y,z,P)$ be a feasible solution for the \lpMEWC or \lpMVWC instance $(G = (V, E), \Tc, \Tt, w)$.
Assuming $\Tc \eps < \frac{1}{\Tc}$, the solution constructed at the end of step $3$ of Algorithm~\ref{alg:weak-coloring-rounding}, $(\hat{x},\hat{y},\hat{z},\hat{P})$, is a $(\frac{1}{1/\Tc - \Tc \eps})$-feasible solution for $(G, \Tc, \Tt, w)$ such that $\cost(\hat{x},\hat{y},\hat{z},\hat{P}) \leq \frac{1}{\eps} \cdot \cost(x,y,z,P)$.
\end{corollary}

\begin{proof}
By Lemma~\ref{lem:step-2}, after step $2$ of Algorithm~\ref{alg:weak-coloring-rounding}, $(\hat{x},\hat{y},\hat{z},\hat{P})$ is a $\frac{1}{1/\Tc - \Tc \eps}$-feasible solution to $(G, \Tc, \Tt, w)$ with cost at most $\frac{1}{\eps} \cdot \cost(x,y,z,P)$.
Furthermore, the only constraint that can be violated by rounding $z_{\set{pq}}$ or $z_p$ down is Constraint~\eqref{cst:hop}.
The constraint is trivially satisfied if some $z_{\set{pq}}$ or $z_p$ has been rounded up or $y_{Tv}$ has been rounded down.
Additionally, in step $2$ of Algorithm~\ref{alg:weak-coloring-rounding}, we set $\hat{P}_{uv} = 1$ in all other cases.
\end{proof}

We have stated that at the end of the first phase of our rounding algorithm (steps $1$--$3$), the algorithm constructs a fractional $(\frac{1}{1/\Tc - \Tc \eps})$-feasible solution such that $\hat{z}$ is integral.
Since, $\hat{z}$ is an integral vector, we can construct a solution $\hat{\editset} := \set{\set{uv} : \hat{z}_{\set{uv}} = 1}$ for edge deletion or $\hat{\editset} := \set{v : \hat{z}_v = 1}$ for vertex deletion as stated at the end of Algorithm~\ref{alg:weak-coloring-rounding}.
Finally, we show that $\hat{\editset}$ is an $(O(1),O(1))$-bicriteria approximation solution for the \bWCN instance $(G, \Tc, \Tt, w)$.

\begin{lemma} \label{lemma:wcnlp-edited}
The edited graph $G \setminus \hat{\editset}$ has weak $\Tc$-coloring number at most $\frac{\Tt}{1/\Tc - \Tc \eps}$.
\end{lemma}

\begin{proof}
This follows directly from the fact that $|\wreach{\Tc}{G \setminus \hat{\editset}}{L}{u}| \leq \sum_{v \in V} \hat{P}_{uv}$ for the optimal ordering $L$.
Since we allow $\hat{x}_{v_1 v_3}$ to be larger than it should be by allowing forward cycles, $\hat{y}_{Tv}$ can also be larger than optimal.
Thus, $\hat{P}_{uv}$ is forced to be larger than the optimal as well for some vertices.
This causes the LP to over-estimate the weak $\Tc$-reachability of each vertex.
\end{proof}

Finally, we have the following theorem.

\begin{theorem} \label{thm:main-weak-coloring}
Assuming $\Tc \eps < 1/\Tc$, there exists a $(\frac{1}{\eps}, \frac{1}{1/\Tc - \Tc \eps})$-bicriteria approximation algorithm for the \bWCN instance $(G, \Tc, \Tt, w)$.
\end{theorem}

\begin{proof}
First we solve \lpMEWC or \lpMVWC for $(G, \Tc, \Tt, w)$ in polynomial time to get an optimal fractional solution $(x,y,z,P)$.
Then, we run Algorithm~\ref{alg:weak-coloring-rounding} to produce $(\hat{x},\hat{y},\hat{z},\hat{P})$ which by Corollary~\ref{cor:step-3} has cost at most $\frac{1}{\eps} \cdot \cost(x,y,z,P)$ and is a $(\frac{1}{1/\Tc - \Tc \eps})$-feasible solution.
By Lemma~\ref{lemma:wcnlp-edited}, the solution $\hat{\editset}$ has weight at most $\frac{1}{\eps}$ times the optimal and produces an edited graph $G \setminus \hat{\editset}$ such that $\wcol{\Tc}{G \setminus \hat{\editset}} \leq \frac{\Tt}{1/\Tc - \Tc \eps}$.
\end{proof}

